Quantitative Analysis of Assertion Violations in Probabilistic Programs

In this work, we consider the fundamental problem of deriving quantitative bounds on the probability that a given assertion is violated in a probabilistic program. We provide automated algorithms that obtain both lower and upper bounds on the assertion violation probability in exponential forms. The main novelty of our approach is that we prove new and dedicated fixed-point theorems which serve as the theoretical basis of our algorithms and enable us to reason about assertion violation bounds in terms of pre and post fixed-point functions. To synthesize such fixed-points, we devise algorithms that utilize a wide range of mathematical tools, including repulsing ranking super-martingales, Hoeffding's lemma, Minkowski decompositions, Jensen's inequality, and convex optimization. On the theoretical side, we provide (i) the first automated algorithm for lower-bounds on assertion violation probabilities, (ii) the first complete algorithm for upper-bounds of exponential form in affine programs, and (iii) provably and significantly tighter upper-bounds than the previous approach of stochastic invariants. On the practical side, we show that our algorithms can handle a wide variety of programs from the literature and synthesize bounds that are several orders of magnitude tighter in comparison with previous approaches.

==> overview-syc.tex <==
\section{An Overview of Our Results}

We focus on \yican{shall we remove this: sound approaches for} deriving probabilistic upper and lower bounds for assertion violation in probabilistic programs.
We first establish our general approach through fixed-point theorems, for which we derive the upper bounds from the least fixed-point theorem,
and introduce a novel fixed-point theorem for deriving the lower bounds.
Then \textit{our algorithm adopts} the template-based method and consider the automated synthesis of \emph{exponential} templates.
For probabilistic upper bounds, we show that exponential templates can be solved exactly through convex programming, thus leading to a \textit{sound and complete} algorithm.
For probabilistic lower bounds, we apply Jensen's inequality to obtain an algorithm that is \textit{sound but incomplete}.

In the following, we present three examples from different application domains, namely tortoise-hare race, concentration bound of termination time and unreliable hardware,
where probabilistic bounds of failure assertions are prominent.

\subsection{Tortoise-Hare Race}
\label{sec:rabbit}


	Consider the following probabilistic program from the background of stochastic invariant~\cite{?}:
	\lstset{language=prog}
	\lstset{tabsize=3}
	\newsavebox{\progrunningexampleb}
	\begin{lstlisting}[mathescape]
	input: $x$:=$40$; $y$:=0;
	while($x\leq 99\land y\leq 99$)do
		if prob($0.5$) then
			$\langle x,y\rangle:=\langle x+1,y+2\rangle$
		else
			$\langle x,y\rangle:=\langle x+1,y\rangle$
	od
	assert($x \geq 100$)
	\end{lstlisting}

	The example presents a scenario of tortoise-hare Race. In the program,
	the variable $x$ represents the turtle's position, while the variable $y$ represents the hare's.
	At each time, the tortoise always proceeds with one unit distance to the destination (i.e., positions beyond $100$), while the lazy hare would either jump for two unit distance or take a rest with equal probability.
	The \textbf{assert} expression at the end indicates the winning condition for the tortoise: if the hare reaches the destination strictly before the tortoise, then the tortoise loses the race and the assertion $x\le 100$ fails, otherwise the tortoise wins and the program terminates normally.
	Our goal is to give an upper bound of the hare's winning probability, that is, to infer an upper bound of the probability that the assertion at the end of the program fails.

Our theory is established via fixed-point theorems. Here we only present an intuitive description.
The core part of our approach is to synthesize a function
$f(x^*,y^*)$ that approximates
the probability of assertion violation when the program starts at the entry point to the while loop and
the initial values of the variables $x,y$ are given as $x^*,y^*$ respectively.
We set up a collection of constraints for every $(x^*, y^*)$ as follows:
\begin{enumerate}
	\item[(1)] $\forall x^*, y^*. f(x^*, y^*)\ge 0$;
	\item[(2)] $\forall x^*. \left(x^* \ge 100 \Rightarrow f(x^*,y^*)=0\right)$;
	\item[(3)] $\forall x^*,y^*. \left(x^*\le 99\land y^*\ge 100 \Rightarrow  f(x^*,y^*)=1\right)$;
	\item[(4)] $\forall x^*,y^*. [(x^*\le 99\land y^*\le 99) \Rightarrow f(x^*,y^*)\ge \frac12f(x^*+1,y^*+2)+\frac12f(x^*+1,y^*)]$.
\end{enumerate}
Informally, the constraint (1) is natural since probability values are always non-negative.
Note that this constraint is also necessary  to apply the Tarski's fixed-point theorem (cf. Theorem \ref{thm:tarski}).
Next, the constraint (2) refers to normal termination without assertion failure, while the constraint (3) corresponds to the case of assertion failure.
Finally, the constraint (4) is the condition applied to the situation where the program does not terminate at the current step, which is
derived from the fixed-point theorem and states that $f(x^*,y^*)$ is a \yican{pre-fixed point}.
Note that the expression $\frac12f(x^*+1,y^*+2)+\frac12f(x^*+1,y^*)$ represents the expected value of the function $f$ after one loop iteration of the program.

By Tarski's fixed-point theorem, if we can find a function $f(x^*, y^*)$ that satisfies the constraints (1)--(4), then this function serves as an upper bound for assertion violation probability for every input $x^*,y^*$.
In this work, we consider that assertion violation probability be small and decrease drastically w.r.t certain amount, for which a suitable choice would be exponential functions.
We follow the template-based method (see e.g.~\cite{?,?,?}) and set up an exponential template $f(x^*,y^*):=\exp(a\cdot x^* + b\cdot y^* + c)$ over points $(x^*, y^*)$ that satisfy the constraint (4) above, with unknown coefficents $a,b,c$ to be solved.
Note that this template specifies that the assertion violation probability decreases exponentially w.r.t the linear expression $a\cdot x^* + b\cdot y^* + c$.
The choice of the coefficients $a,b,c$ needs to fulfill the constraint (1)--(4), while simultaneously minimizing $f(x_{\mathrm{init}}, y_{\mathrm{init}})$ for a given pair of fixed initial values $x_{\mathrm{init}}, y_{\mathrm{init}}$ for variables $x,y$ respectively.
we need to minimize the probability for initial state.
Thus, we reduce the solution of the unknown coefficients $a,b,c$ into an optimization problem.
Taking $(x_{\mathrm{init}}, y_{\mathrm{init}}):=(40,0)$ and $f(x^*, y^*; a,b,c):=\exp(a\cdot x^* + b\cdot y^* + c)$,
we derive the following optimization problem for the constraint (4):
$$\textbf{objective function:}~~~~~ \min_{a,b,c} \exp(40\cdot a + 0\cdot b + c)$$
\textbf{subject to:}

\begin{align*}
& \forall x^*, y^*. [(40 \le x^*\le 98 \land 0\le y^*\le 97)\Rightarrow \\
& \quad(\frac12\cdot f(x^*+1, y^*+2; a,b,c)+ \frac12\cdot f(x^*+1, y^*; a,b,c) \\
& \qquad\le f(x^*, y^*; a,b,c))] \\
& \\
& \forall x^*, y^*. [(40\le x^*\le 98 \land 98\le y^*\le 99)\Rightarrow \\
& \quad\frac12 + \frac12\cdot f(x^*+1, y^*; a,b,c) \le f(x^*, y^*; a,b,c)] \\
& \\
& \forall x^*, y^*. [(x^*=99 \land 0\le y^*\le 99)\Rightarrow 0\le f(x^*, y^*; a,b,c)]\\
\end{align*}


The first constraints above specifies the situation $40 \le x^*\le 98 \wedge 0\le y^*\le 97$ where the program will not terminate after one loop iteration.
The second specifies the situation $40\le x^*\le 98 \land 98\le y^*\le 99$ where the program may end with the hare winning after one loop iteration.
The third specifies the situation $x^*=99 \land 0\le y^*\le 99$ where the program will end with the tortoise winning after one loop iteration.
In general, it is difficult to solve such kind of optimization problems where the constraints are univerally-quantified and involve exponential terms.
Suprisingly, we show that a large class of optimization problems of this kind (including the optimization problem above) can be exactly solved through convex programming.
By solving this optimization problem, we derive that $a\approx-1.19,b\approx 4.26,c\approx 31.79$, and the minimum is $\approx \exp(-15.697)\approx 1.524\cdot 10^{-7}$. \yican{yican: to compare hoeffding's inequality/Precise result here, precise is $2.632\cdot 10^{-8}$, hoeffding is $6.507\cdot 10^{-7}$}

\yican{yican: limitation}.
\yican{yican: compare two algorithm here}.


\subsection{Concentration Bound of Termination Time}

Concentration-bound analysis of termination time is a fundamental problem in probabilistic-program analysis.
The task is to have rapidly-decreasing upper bounds for the probability that a probabilistic program does not terminate within a given amount of execution steps.
To model termination in our framework,
we introduce a fresh variable $t$ to record the running time whose value is initialized to $0$,
add the statement $t:=t+1$ at each place where the number of execution steps is supposed to increase by one,
and insert the assertion $\mathbf{\mathrm{assert}}(t<r)$ at appropriate places, where $r$ is either a user-specified amount or a fresh variable indicating that
the probabilistic program of concern should terminate within $r$ steps with high probability.
To illustrate the idea, we take a simple example of an asymmetric random walk below:

	\lstset{language=prog}
	\lstset{tabsize=3}
	\begin{lstlisting}[mathescape]

	input: $x$:=$0$; $t$:=$0$;
	while($x\leq 99$)do
		switch do
			prob($0.75$):$\langle x,t\rangle$:=$\langle x+1,t+1\rangle$
			prob($0.25$):$\langle x,t\rangle$:=$\langle x-1,t+1\rangle$
		od
		assert($t\le 500$)
	od
	\end{lstlisting}

	In the program, the variable $x$

Our goal is to infer the tail bound of the running time of a random walk.
	At each iteration, with probability $p$ the current update of $x$ fails, otherwise $x$ increments with probability $0.75$, or decrements with probability $0.25$.
	We use the method above to transform this task into a case in \textit{QRA}.

Similarly to the previously example, we need to synthesize function $f(x,t)$ that always overestimates the probability:
\begin{enumerate}
	\item[(0)] $\forall x,t$, $f(x,t)\ge 0$
	\item[(1)] $\forall -\infty< x< +\infty\land t\ge 501, f(x,t)=1$
	\item[(2)] For $x=100\land t\le 500, f(x,t)=0$
	\item[(3)] For $t=500\land \forall x\le 99, f(x,t)\ge 1$
	\item[(4)] For $x=99\land \forall t\le 499$, $$f(x,t) \ge 0.25\cdot f(x-1,t+1) + 0.75\cdot 0$$
	\item[(5)] $\forall t\le 499\land x\le 98$,
	$$f(x,t) \ge 0.25\cdot f(x-1,t+1) + 0.75\cdot f(x+1,t+1)$$
\end{enumerate}

By solving this system, we derive that $a\approx -0.351, b\approx 0.124, c\approx -27.404$, and the result is $\approx \exp(-27.754)\approx 8.85\cdot 10^{-13}$


\subsection{Unreliable hardware}
\label{sec:hardware}
Now we present another example.
Consider an unreliable hardware, where any computation on this hardware would fail with probability about $p:=10^{-7}$.
Our goal is to derive the lower bound of the probability that a program executes correctly. Concretely, we consider the following program:

\begin{example}[\textit{Unreliable Hardware}]\label{ex:unrel}
	\lstset{language=prog}
	\lstset{tabsize=3}
	\begin{lstlisting}[mathescape]

	input: $x$:=$1$;
	while($x\leq 99$)do
		switch do
			prob($p$):exit
			prob($0.75\cdot (1-p)$):$x$:=$x+1$
			prob($0.25\cdot (1-p)$):$x$:=$x-1$
		od
	od
	assert($true$)
	\end{lstlisting}

	The program simulates the one-dimensional random walk, presented in \ref{ex:rdwalk}, on an unreliable hardware. At each time there are probability $p$ that the arithmetic operation fails. The assert expression in the end represents that if there is \textit{no hardware failure} during the whole computation, then the assert expression fails, otherwise the program would terminate.
	Since we are interested in the lower bound of the probability that there is no hardware error, we need to infer the probability that the program terminates with assert fails.
	\end{example}


Contrary with previous examples, since we need to infer lower bound, we need to synthesize function $f(x_0)$ that always underestimates the probability:
\begin{enumerate}
	\item[(0)] $\forall x_0$, $f(x_0)\le 1$
	\item[(1)] For $x_0\ge 100, f(x_0)=1$
	\item[(2)] For $x_0\le 99$, $$f(x_0)\leq 0.75 \cdot (1-p)\cdot  f(x_0+1) + 0.25\cdot (1-p) \cdot f(x_0-1) + p\cdot 0$$
\end{enumerate}

(0) is natural since probability is no more than $1$, it is also a necessary condition to guarantee the uniqueness of fixed-point, thus we could apply Theorem \ref{thm:tarski} to infer lower bound. The detail of this is shown in Theorem \ref{thm:uniq}. (1) is for assertion failure. Finally, (2) represents the case that the program continues execution.


We still set up a template $f(x_0):=\exp(a\cdot x_0  + b)$ for $x_0\le 99$. Plugging in this template into (0)-(2), we derive constraints for $a,b$, and solve the optimization problem below:
$$\max_{a,b} \exp(a\cdot 1  + b)$$
Such that:
\begin{enumerate}
	\item[(I)] $\forall x_0\le 99$, $a\cdot x_0 + b\le 0$
	\item[(II)] $\forall x_0\le 98$,
	$$\exp(a\cdot x_0 + b)\leq
	\begin{matrix}
	0.75\cdot (1-p)\cdot \exp(a\cdot (x_0 + 1) + b)\\
	 + 0.25 \cdot (1-p) \cdot \exp(a\cdot (x_0-1) + b)
	\end{matrix}
	$$
	\item[(III)] $\forall x_0=99$,
	$$\exp(a\cdot 99 + b)\leq
	0.75\cdot (1-p)
	 + 0.25 \cdot (1-p) \cdot \exp(a\cdot 98 + b)
	$$
\end{enumerate}

We do transposition on (II), by dividing $\exp(a\cdot x_0 + b)$ on both side, we have:
$$0.75\cdot (1-p)\cdot \exp(a) + 0.25\cdot (1-p)\cdot \exp(-a) \ge 1$$

Since this does not represent a convex set on $\Rset^2$, it is a non-convex and non-linear optimization problem. Hence it is considered to be hard in general. In this paper, we present use Jensen's inequality to relax exponential constraints to linear ones:
\begin{itemize}
	\item (II) is satisfied if $$0.75\cdot a + 0.25\cdot(-a) \ge \ln\left(\frac{1}{1-p}\right)$$
	\item (III) is satisfied if $$0.75\cdot (-99\cdot a -b) + 0.25 \cdot(-a) \ge \ln\left(\frac{1}{1-p}\right)$$
\end{itemize}

After these transformations, note that maximize $\exp(a+b)$ is equivalent to maximize $a+b$, the problem become a linear programming problem, thus could be solved efficiently.

By calculation, we have $a\approx 2\cdot 10^{-7},b\approx 2\cdot 10^{-5}$, Hence the result is $\approx \exp(-1.98\cdot 10^{-5}) \approx 0.99998$.

\yican{yican: a remark here to compare with Rely/Hsu's paper}

